Combinatorial Multi-Armed Bandit and Its Extension to Probabilistically Triggered Arms

We define a general framework for a large class of combinatorial multi-armed bandit (CMAB) problems, where subsets of base arms with unknown distributions form super arms. In each round, a super arm is played and the base arms contained in the super arm are played and their outcomes are observed. We further consider the extension in which more based arms could be probabilistically triggered based on the outcomes of already triggered arms. The reward of the super arm depends on the outcomes of all played arms, and it only needs to satisfy two mild assumptions, which allow a large class of nonlinear reward instances. We assume the availability of an offline (\alpha,\beta)-approximation oracle that takes the means of the outcome distributions of arms and outputs a super arm that with probability {\beta} generates an {\alpha} fraction of the optimal expected reward. The objective of an online learning algorithm for CMAB is to minimize (\alpha,\beta)-approximation regret, which is the difference between the \alpha{\beta} fraction of the expected reward when always playing the optimal super arm, and the expected reward of playing super arms according to the algorithm. We provide CUCB algorithm that achieves O(log n) distribution-dependent regret, where n is the number of rounds played, and we further provide distribution-independent bounds for a large class of reward functions. Our regret analysis is tight in that it matches the bound of UCB1 algorithm (up to a constant factor) for the classical MAB problem, and it significantly improves the regret bound in a earlier paper on combinatorial bandits with linear rewards. We apply our CMAB framework to two new applications, probabilistic maximum coverage and social influence maximization, both having nonlinear reward structures. In particular, application to social influence maximization requires our extension on probabilistically triggered arms.

==> icmlreference.tex <==

\begin{thebibliography}{22}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi
\setlength{\itemsep}{0mm}
\bibitem[Anantharam et~al.(1987{\natexlab{a}})Anantharam, Varaiya, and
  Walrand]{AVW87a}
Anantharam, V., Varaiya, P., and Walrand, J.
\newblock Asymptotically efficient allocation rules for the multiarmed bandit
  problem with multiple plays --- {P}art {I}: i.i.d. rewards; {P}art {II}: {M}arkovian rewards.
\newblock \emph{IEEE Transactions on Automatic Control}, AC-32\penalty0
  (11):\penalty0 968--982, 1987{\natexlab{a}}.

\bibitem[Audibert et~al.(2009)Audibert, Bubeck, and Lugosi]{Audibert2009}
Audibert, J.-Y., and Bubeck, S.
\newblock Minimax policies for adversarial and stochastic bandits.
\newblock In \emph{COLT}, 2009.

\bibitem[Audibert et~al.(2011)Audibert, Bubeck, and Lugosi]{Audibert2011}
Audibert, J., Bubeck, S., and Lugosi, G.
\newblock Minimax policies for combinatorial prediction games.
\newblock In \emph{COLT}, 2011.

\bibitem[Auer et~al.(2002{\natexlab{a}})Auer, Cesa-Bianchi, and
  Fischer]{AuerCF02}
Auer, P., Cesa-Bianchi, N., and Fischer, P.
\newblock Finite-time analysis of the multiarmed bandit problem.
\newblock \emph{Machine Learning}, 47\penalty0 (2-3):\penalty0 235--256,
  2002{\natexlab{a}}.

\bibitem[Auer et~al.(2002{\natexlab{b}})Auer, Cesa-Bianchi, Freund, and
  Schapire]{AuerCFS02}
Auer, P., Cesa-Bianchi, N., Freund, Y., and Schapire, R.~E.
\newblock The nonstochastic multiarmed bandit problem.
\newblock \emph{SIAM J. Comput.}, 32\penalty0 (1):\penalty0 48--77,
  2002{\natexlab{b}}.

\bibitem[Berry \& Fristedt(1985)Berry and Fristedt]{BF85}
Berry, D. and Fristedt, B.
\newblock \emph{Bandit problems}.
\newblock Chapman and Hall, 1985.

\bibitem[Bubeck et~al.(2012)Bubeck, Cesa-Bianchi, and Kakade]{Bubeck12}
Bubeck, S.,  Cesa-Bianchi, N., and  Kakade, S.~M.
\newblock Towards Minimax Policies for Online Linear Optimization with Bandit Feedback.
\newblock In \emph{COLT}, 2012.

\bibitem[Caro \& Gallien(2007)Caro and Gallien]{CG07}
Caro, F. and Gallien, J.
\newblock Dynamic assortment with demand learning for seasonal consumer goods.
\newblock \emph{Management Science}, 53, 276--292, 2007.

\bibitem[Cesa-Bianchi \& Lugosi(2009)Cesa-Bianchi and Lugosi]{CL09}
Cesa-Bianchi, N. and Lugosi, G.
\newblock Combinatorial bandits.
\newblock Journal of Computer and System Sciences, 78(5), 2011.

\bibitem[Chen et~al.(2013)]{CWY13}
Chen, W., Wang, Y., and Yuan, Y.
\newblock Combinatorial multi-armed bandit: general framework, results, and applications.
\newblock In \emph{ICML}, 2013.

\bibitem[Gai et~al.(2010)Gai, Krishnamachari, and Jain]{GaiKJ10}
Gai, Y., Krishnamachari, B., and Jain, R.
\newblock Learning multiuser channel allocations in cognitive radio networks: A
  combinatorial multi-armed bandit formulation.
\newblock In \emph{DySPAN}, 2010.

\bibitem[Gai et~al.(2012)Gai, Krishnamachari, and Jain]{Yi2012}
Gai, Y., Krishnamachari, B., and Jain, R.
\newblock Combinatorial network optimization with unknown variables:
  Multi-armed bandits with linear rewards and individual observations.
\newblock \emph{IEEE/ACM Transactions on Networking}, 20, 2012.

\bibitem[Garivier \& Capp{\'e}(2011)Garivier and Capp{\'e}]{Garivier2011}
Garivier, A. and Capp{\'e}, O.
\newblock The {KL-UCB} algorithm for bounded stochastic bandits and beyond.
\newblock In \emph{COLT}, 2011.

\bibitem[Hazan \& Kale(2009)Hazan and Kale]{Hazan2009}
Hazan, E. and Kale, S.
\newblock Online submodular minimization.
\newblock In \emph{NIPS}, 2009.

\bibitem[Kakade et~al.(2009)Kakade, Kalai, and Ligett]{Kakade2009}
Kakade, S.~M., Kalai, A.~T., and Ligett, K.
\newblock Playing games with approximation algorithms.
\newblock \emph{SIAM Journal on Computing}, 39\penalty0 (3):\penalty0
  1088--1106, 2009.

\bibitem[Kempe et~al.(2003)Kempe, Kleinberg, and Tardos]{kempe03}
Kempe, D., Kleinberg, J.~M., and Tardos, {\'E}.
\newblock Maximizing the spread of influence through a social network.
\newblock In \emph{KDD}, 2003.

\bibitem[Lai \& Robbins(1985)Lai and Robbins]{LaiRobbins85}
Lai, T.~L. and Robbins, H.
\newblock Asymptotically efficient adaptive allocation rules.
\newblock \emph{Advances in Applied Mathematics}, 6:\penalty0 4--22, 1985.

\bibitem[Liu et~al.(2011)Liu, Liu, and Zhao]{LiuLZ11}
Liu, H., Liu, K., and Zhao, Q.
\newblock Logarithmic weak regret of non-bayesian restless multi-armed bandit.
\newblock In \emph{ICASSP}, 2011.
\bibitem[Liu \& Zhao(2012)Liu and Zhao]{Liu2012}
Liu, K. and Zhao, Q.
\newblock Adaptive shortest-path routing under unknown and stochastically
  varying link states.
\newblock \emph{Arxiv preprint arXiv:1201.4906}, 2012.

\bibitem[Mannor \& Shamir(2011)Mannor and Shamir]{Mannor2011}
Mannor, S., and Shamir, O.
\newblock From Bandits to Experts: On the Value of
Side-Observations.
\newblock In \emph{NIPS}, 2011.


\bibitem[Nemhauser et~al.(1978)Nemhauser, Wolsey, and Fisher]{NWF78}
Nemhauser, G., Wolsey, L., and Fisher, M.
\newblock An analysis of the approximations for maximizing submodular set
  functions.
\newblock \emph{Mathematical Programming}, 14:\penalty0 265--294, 1978.

\bibitem[Radlinski et~al.(2008)Radlinski, Kleinberg, and
  Joachims]{Radlinski2008}
Radlinski, F., Kleinberg, R., and Joachims, T.
\newblock Learning diverse rankings with multi-armed bandits.
\newblock In \emph{ICML}, 2008.

\bibitem[Streeter et~al.(2009)Streeter, Golovin, and Krause]{Streeter2009}
Streeter, M., Golovin, D., and Krause, A.
\newblock Online learning of assignments.
\newblock In \emph{NIPS}, 2009.

\bibitem[Streeter \& Golovin(2008)Streeter and Golovin]{Streeter2008}
Streeter, M. and Golovin, D.
\newblock An online algorithm for maximizing submodular functions.
\newblock In \emph{NIPS}, 2008.

\bibitem[Sutton \& Barto(1998)Sutton and Barto]{SB98}
Sutton, R. and Barto, A.
\newblock \emph{Reinforcement learning, an introduction}.
\newblock MIT Press, 1998.

\bibitem[Vazirani (2004)Vazirani]{Vazirani04}
Vazirani, V.~V.
\newblock \emph{Approximation Algorithms}
\newblock Springer, 2004

\end{thebibliography}
